Uncoupled Regression from Pairwise Comparison Data

Uncoupled regression is the problem to learn a model from unlabeled data and the set of target values while the correspondence between them is unknown. Such a situation arises in predicting anonymized targets that involve sensitive information, e.g., one's annual income. Since existing methods for uncoupled regression often require strong assumptions on the true target function, and thus, their range of applications is limited, we introduce a novel framework that does not require such assumptions in this paper. Our key idea is to utilize pairwise comparison data, which consists of pairs of unlabeled data that we know which one has a larger target value. Such pairwise comparison data is easy to collect, as typically discussed in the learning-to-rank scenario, and does not break the anonymity of data. We propose two practical methods for uncoupled regression from pairwise comparison data and show that the learned regression model converges to the optimal model with the optimal parametric convergence rate when the target variable distributes uniformly. Moreover, we empirically show that for linear models the proposed methods are comparable to ordinary supervised regression with labeled data.

==> Taylor_bregman.tex <==
The first idea is to approximate $y$ from $F_Y$. From Taylor expansion at $y=y_0$, we have
\begin{align*}
    &F_Y(y) = F_Y(y_0) + f_Y(y_0)(y-y_0) + O((y-y_0)^2) \\
    &\therefore y = \frac{F_Y(y) - F_Y(y_0) + y_0f_Y(y_0)}{f_Y(y_0)} + O((y-y_0)^2) .
\end{align*}
Using this approximation, loss function can be written as follows.
\begin{lem}\label{lem:Taylor-loss-difference}
Let $R_T(h)$ be the loss defined as 
\begin{align*}
    R_T(h) &= \mathfrak{C} - \frac{\lambda}{2f_Y(y_0)} \expect{\vec{X}^+}{\phi'(h(\vec{X}^+))} +  \frac{1-\lambda}{2f_Y(y_0)} \expect{\vec{X}^-}{\phi'(h(\vec{X}^-))} \\
    &\quad -\expect{\vec{X}}{\left(y_0 + \frac{1-\lambda - F_Y(y_0)}{f_Y(y_0)} - h(\vec{X})\right)\phi'(h(\vec{X}))+\phi(h(\vec{X}))}.
\end{align*}
Now, we denote $\mathrm{Err}_1$ be the maximum error involved in the first-order Taylor approximation, defined as
\begin{align*}
    \mathrm{Err}_1(y_0) = \max_{y\in\mathcal{Y}} \left|y - \frac{F_Y(y) - F_Y(y_0) + y_0f_Y(y_0)}{f_Y(y_0)}\right|,
\end{align*}
and we assume $\mathrm{Err}_1(y_0) \leq \infty$. Then, for any constants $y_0 \in \mathcal{Y}$ and $\lambda \in \mathbb{R}$ ,  we have
\begin{align*}
    |R(h) - R_T(h)| \leq \mathrm{Err}_1(y_0) \expect{X}{|\phi'(\vec{X})|}.
\end{align*}
for all $h \in \mathcal{H}$.
\end{lem}

Therefore, minimizing following empirical risk yields the lower loss.

\begin{align}
    \hat{R}_T(h) &= \mathfrak{C} -\frac{\lambda}{2n_\rank f_Y(y_0)} \sum_{\vec{x}^+_i \in \mathcal{D}^+_\rank} \phi'(h(\vec{x}_i^+)) +  \frac{1-\lambda}{2 n_\rank f_Y(y_0)}\sum_{\vec{x}^-_i \in \mathcal{D}^-_\rank} \phi'(h(\vec{x}_i^-)) \notag\\
    &\quad - \frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} \left\{\left( - y_0 + \frac{1-\lambda - F_Y(y_0)}{f_Y(y_0)} - h(\vec{x}_i)\right)\phi'(h(\vec{x_i})) + \phi(h(\vec{x}_i))\right\}. \label{eq:empirical-Taylor-bregman-decomposition}
\end{align}

Using the same discussion as Theorem~\ref{thm:uniform-generalization-bound}, we have
\begin{thm}\label{thm:uniform-taylor-bound}
    Assume that $\phi'(h(\vec{x}))$ is bounded for all $\vec{x}\in\mathcal{X}$.  Then we have 
\begin{align*}
    R(\hat{h}_T) \leq R(h^*) + O\left(\sqrt{\frac{\log 1/\delta}{n_\unlabeled}}\right) + O\left(\sqrt{\frac{\log 1/\delta}{n_\rank}}\right) + 2\mathrm{Err}_1(y_0) \expect{X}{|\phi'(\vec{X})|}
\end{align*}
with probability $1-4\delta$, where $h^*, \hat{h}_T$ is the minimizer of \eqref{eq:bregman-decomposition} and \eqref{eq:empirical-Taylor-bregman-decomposition}, respectively.
\end{thm}

Although we can only obtain first-order approximation from this pairwisely compared data, we can gain more accurate approximation of bregman divergence if we have additional comparison data. Let $\vec{X}^{(1)},\vec{X}^{(2)},\dots, \vec{X}^{(m)}$ be the random variable, where $(\vec{X}^{(k)}, Y^{(k)})$ follows the joint distribution $P(\vec{X},Y)$ and we permute them so that $Y^{(1)} \geq Y^{(2)} \geq  \cdots \geq Y^{(m)}$. Note that $(\vec{X}^+,\vec{X}^-)$ are the special case of $m=2$. Then, from the similar discussion, the PDF $f_{\vec{X}^{(k)}}$ of $\vec{X}^{(k)}$ can be written as 
\begin{align*}
    f_{\vec{X}^{(k)}}(\vec{x}) = \frac{1}{Z^{(i)}} \int f_{\vec{X},Y}(\vec{x},y) (F_Y(y))^{m-k} (1-F_Y(y))^{k-1}\intd y
\end{align*}
for some normalizing constant $Z^{(i)}$. Now, we have $m$ different distributions, which yields $(m-1)$-th order approximation of $R(h)$. 

\begin{lem}
Let $(b_0,b_1, \cdots, b_m)$ be the one of the solutions of the following linear programming.
\begin{align*}
    \begin{bmatrix}
    1&a_{1,0}& a_{2,0}& \dots & a_{m,0}\\
    0&a_{1,1}& a_{2,1}& \dots & a_{m,1}\\
    0&a_{1,2}& a_{2,2}& \dots & a_{m,2}\\
    \vdots& \vdots& \vdots & \ddots & \vdots\\
    0& a_{1,m-1}& a_{2,m-1}& \dots & a_{m,m-1}\\
    \end{bmatrix}
    \begin{bmatrix}
    b_0\\
    b_1\\
    b_2\\
    \vdots\\
    b_{m}
    \end{bmatrix}
    =
    \begin{bmatrix}
    0\\
    1\\
    0\\
    \vdots\\
    0
    \end{bmatrix},
\end{align*}
where $a_{k,l}$ is the $l$-th Taylor series of $(F_Y(y))^{m-k} (1-F_Y(y))^{k-1}$, defined as
\begin{align*}
    a_{k,l} = \lim_{y\to y_0} \frac{(F_Y(y))^{m-k} (1-F_Y(y))^{k-1} - \sum_{i=0}^{l-1} a_{k,i}(y-y_0)^i }{(y-y_0)^l}.
\end{align*}
Then, the loss $R^{(m-1)}_T(h)$ defined as 
\begin{align*}
    R^{(m-1)}_T(h) &= \mathfrak{C} - \expect{\vec{X}}{\phi(h(\vec{X})) + h(\vec{X})\phi'(h(\vec{X}))}\\
         &\quad -(y_0 + b_0)\expect{\vec{X}}{\phi'(h(\vec{X}))} - \sum_{i=1}^m b_iZ^{(i)}\expect{\vec{X}^{(i)}}{\phi'(h(\vec{X}^{(i)}))}
\end{align*}
satisfies 
\begin{align*}
    |R(h) - R^{(m-1)}_T(h)| \leq \mathrm{Err}_{m-1}(y_0) \expect{X}{|\phi'(\vec{X})|}.
\end{align*}
for all $h \in \mathcal{H}$, where
\begin{align*}
    \mathrm{Err}_{m-1}(y_0) = \argmax_{y\in\mathcal{Y}} \left|y - \left(y_0 + b_0 + \sum_{k=1}^m b_k (F_Y(y))^{m-k} (1-F_Y(y))^{k-1}\right)\right|.
\end{align*}
\end{lem}

\begin{comment}
\begin{lem}
Let $(c_0,c_1,c_2,c_3)$ be the one of the solutions of the following linear programming.
\begin{align*}
    \begin{bmatrix}
    1&(F_0)^2& F_0 - (F_0)^2 & 1 - 2F_0 + (F_0)^2\\
    0& 2F_0f_0& f_0 - 2F_0f_0& 2F_0f_0 - 2f_0\\
    0& F_0f'_0+(f_0)^2& \frac{f'_0}2-F_0f'_0+(f_0)^2&-f'_0+F_0f'_0+(f_0)^2\\
    \end{bmatrix}
    \begin{bmatrix}
    c_0\\
    c_1\\
    c_2\\
    c_3\\
    \end{bmatrix}
    =
    \begin{bmatrix}
    0\\
    1\\
    0
    \end{bmatrix},
\end{align*}
where $F_0 = F_Y(y_0), f_0 = f_Y(y_0), f'_0 = f'_Y(y_0)$ for some $y_0\in\mathcal{Y}$. Then, the loss $R^{(3)}_T(h)$ defined as 
\begin{align*}
    R^{(3)}_T(h) &= \mathfrak{C} - \expect{\vec{X}}{\phi(h(\vec{X})) + h(\vec{X})\phi'(h(\vec{X}))}\\
         &\quad -(y_0 + c_0)\expect{\vec{X}}{\phi'(h(\vec{X}))} - \sum_{i=1}^3 c_iZ^{(i)}\expect{\vec{X}^{(i)}}{\phi'(h(\vec{X}^{(i)}))}
\end{align*}
satisfies 
\begin{align*}
    |R(h) - R^{(3)}_T(h)| \leq \mathrm{Err}_2(y_0) \expect{X}{|\phi'(\vec{X})|}.
\end{align*}
for all $h \in \mathcal{H}$, where
\begin{align*}
    \mathrm{Err}_2(y_0) = \argmax_{y\in\mathcal{Y}} \left|y - \left(y_0 + c_0 + \sum_{k=1}^3 c_k (F_Y(y))^{3-k} (1-F_Y(y))^{k-1}\right)\right|.
\end{align*}
\end{lem}
\end{comment}



\begin{comment}
    \begin{bmatrix}
    1&(F_Y(y_0))^2& F_Y(y_0) - (F_Y(y_0))^2 & 1 - 2F_Y(y_0) + (F_Y(y_0))^2\\
    0& 2F_Y(y_0)f_Y(y_0)& f_Y(y_0) - 2F_Y(y_0)f_Y(y_0)& 2F_Y(y_0)f_Y(y_0) - 2f_Y(y_0)\\
    0& F_Y(y_0)f'_Y(y_0)+(f_Y(y_0))^2& \frac{f'_Y(y_0)}2-F_Y(y_0)f'_Y(y_0)+(f_Y(y_0))^2&-f'_Y(y_0)+F_Y(y_0)f'_Y(y_0)+(f_Y(y_0))^2\\
    \end{bmatrix}
\end{comment}
    

==> general_case.tex <==
We used the fact $F_Y(y) = y$ in the discussion in the previous section, which does not hold in general. In such a case, we cannot express $\expect{\vec{X},Y}{Y\phi'(h(\vec{X}))}$ in terms of the linear combination of $\expect{\vec{X}}{\phi'(h(\vec{X}))}, \expect{\vec{X}^-}{\phi'(h(\vec{X}^-))}$ and $\expect{\vec{X}^+}{\phi'(h(\vec{X}^+))}$, and thus we cannot directly construct an unbiased estimator of \eqref{eq:expected_loss} from information that we have access to. In this section, we propose two methods for this general setting. One is to transform target variable so that it marginally distributes uniformly, and the other is to use a linear combination of $\expect{\vec{X}}{\phi'(h(\vec{X}))}, \expect{\vec{X}^-}{\phi'(h(\vec{X}^-))}$ and $\expect{\vec{X}^+}{\phi'(h(\vec{X}^+))}$ to approximate $\expect{\vec{X},Y}{Y\phi'(h(\vec{X}))}$. Although we prove that both methods are not consistent, i.e. the loss of learned regression function does not converge to the minimal loss as the size of data increases, they exhibits competitive empirical performances with an ordinary ``coupled'' regression method, as shown later.
 
%When the marginal distribution of target variables is not uniform, we cannot directly minimize the expected loss since $F_Y(y) \neq y$. However, we can still approximate the Bregman divergence or minimize the Bregman divergence between CDF. In this section, we discuss these methods and derive the generalization error bounds for each method.

\subsection{Minimization of Bregman Divergence between CDF}

\input{CDF_bregman.tex}

\subsection{Approximation by Linear Combination}

%\input{Taylor_bregman.tex}
\input{Linear_Approximation.tex}


==> listwise.tex <==
We show that we can further obtain a accurate regression function if ranking data contains more comparisons, which is called \textit{listwise ranking data} \citep{Cao2007}. Let $\vec{X}^{(1)},\vec{X}^{(2)},\dots, \vec{X}^{(m)}$ be the random variables where $(\vec{X}^{(k)}, Y^{(k)})$ follows the joint distribution $P(\vec{X},Y)$, which are permuted so that $Y^{(1)} \geq Y^{(2)} \geq  \cdots \geq Y^{(m)}$. Note that $(\vec{X}^+,\vec{X}^-)$ are the special case of $m=2$. Then, from the similar discussion, the PDF $f_{\vec{X}^{(k)}}$ of $\vec{X}^{(k)}$ can be written as 
\begin{align}
    f_{\vec{X}^{(k)}}(\vec{x}) = \frac{1}{Z^{(k)}} \int f_{\vec{X},Y}(\vec{x},y) (F_Y(y))^{m-k} (1-F_Y(y))^{k-1}\intd y \label{eq:X-listwise-distribtion}
\end{align}
for some normalizing constant $Z^{(k)}$. Now we can build an approximation of risk $R$ with the same discussion as in the pairwise comparison data.

\begin{thm}\label{thm:listwise-bregman-approximation}
Let $\mathcal{D}_\List = \{(\vec{x}_i^{(1)}, \dots, \vec{x}_i^{(m)})\}_{i=1}^{n_\List}$ be  listwise ranking data and $\hat{R}^{(m)}_\linear(h; w_1,\dots,w_m)$ be
\begin{align*}
    \hat{R}^{(m)}_\linear(h; w_1,\dots,w_m) &= \mathfrak{C} - \frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} \phi(h(\vec{x}_i)) - h(\vec{x}_i)\phi'(h(\vec{x}_i)) \\
    &\quad~~~~~~ -  \frac{1}{n_\List} \sum_{k=1}^m \sum_{\vec{x}^{(k)}_i \in \mathcal{D}_\List}  w_k\phi'(h(\vec{x}_i^{(k)})), 
\end{align*}
Then, with the same condition in Theorem~\ref{thm:uniform-taylor-bound}, we have 
\begin{align*}
    R(\hat{h}^{(m)}_\linear) \leq R(h^*) + O\left(\sqrt{\frac{\log 1/\delta}{n_\unlabeled}}\right) + O\left(\sqrt{\frac{\log 1/\delta}{n_\List}}\right) + M\mathrm{Err}^{(m)}(w_1,\dots,w_m)
\end{align*}
with probability $1-(m+1)\delta$, where $h^*$, $\hat{h}^{(m)}_\linear$ are the minimizers of risks $R$ and $\hat{R}^{(m)}_\linear$ in $\mathcal{H}$, respectively, and $\mathrm{Err}^{(m)}(w_1,\dots,w_m)$ is the error in the approximation denoted as
\begin{align*}
    \mathrm{Err}^{(m)}(w_1,\dots,w_m) = \expect{Y}{\left| Y - \sum_{k=1}^m \frac{w_k}{Z^{(k)}} (F_Y(y))^{m-k} (1-F_Y(y))^{k-1}\right|}.
\end{align*}
\end{thm}
The proof can be found in Appendix~\ref{sec:proof-of-listwise-bregman-approximation}. Again, as in the case of pairwise comparison data, we can introduce an free parameter $\lambda$ to reduce the variance of $\hat{R}^{(m)}_\linear$, which is discussed in Appendix \textcolor{red}{TODO:Reference}. We can expect $\mathrm{Err}^{(m)}(w_1,\dots,w_m)$ decreases as $m$ increases since we can employ higher order of $F_Y(y)$ in the approximation.

==> uniform_case.tex <==
In this section, we consider the case where the marginal distribution of the target variables is the uniform distribution on $[0,1]$. In this case, we can easily construct an unbiased estimator of \eqref{eq:expected_loss} for any Bregman divergence.

From the definition of the Bregmain divergence, we have
\begin{align}
    R(h) = \expect{Y}{\phi(Y)} - \expect{\vec{X}}{\phi(h(\vec{X})) - h(\vec{X})\phi'(h(\vec{X}))} -  \expect{\vec{X},Y}{Y\phi'(h(\vec{X}))}. \label{eq:bregman-divergence-trivial-decompose}
\end{align}
In this decomposition, the last term is the only problematic part in uncoupled regression since it is required to calculate the expectation on the joint distribution.
Note that the first term can be regarded as a constant since it does not depend on regression function $h$ and the second term can be empirically approximated by $\mathcal{D}_\unlabeled$. 
Below, we show that the last term can be expressed in terms of pairwise ranking data when target variables are distributed uniformly.

\begin{lem}\label{lem:X_compare_distribution}
    Let $f_{\vec{X}^+}, f_{\vec{X}^-}$ be the probability density functions (PDF) of $P(X^+), P(X^-)$, respectively. Then, we have
    \begin{align*}
        f_{\vec{X}^+}(\vec{x}) = 2\int f_{\vec{X},Y}(\vec{x}, y) F_Y(y)\intd y,~~~f_{\vec{X}^-}(\vec{x}) = 2\int f_{\vec{X},Y}(\vec{x}, y) (1-F_Y(y))\intd y,
    \end{align*}
    where $f_{\vec{X},Y}(\vec{x}, y)$ is the PDF of $P(\vec{X},Y)$ and  $F_Y(y)$ is the CDF of  $P(Y)$. Therefore, when target $Y$ is distributed uniformly, which means $F_Y(y) = y$, we have
    \begin{align*}
        \! \expect{\vec{X},Y}{Y\phi'(h(\vec{X}))} =  \frac{1-\lambda}{2} \expect{\vec{X}^+}{\phi'(h(\vec{X}^+))} - \frac{\lambda}{2} \expect{\vec{X}^-}{\phi'(h(\vec{X}^-))} + \lambda \expect{\vec{X}}{\phi'(h(\vec{X}))}
    \end{align*}
    for all $\lambda \in \mathbb{R}$.
\end{lem}

The proof can be found in Appendix \textcolor{red}{(TODO:Reference)}. From Lemma~\ref{lem:X_compare_distribution} and \eqref{eq:bregman-divergence-trivial-decompose}, we can construct an unbiased estimator $\hat{R}$ of \eqref{eq:expected_loss} as follows.
\begin{align}
    \hat{R}(h) &= \mathfrak{C} - \frac{1}{2n_\rank}\sum_{\vec{x}^+_i, \vec{x}^-_i \in \mathcal{D}_\rank}  (1-\lambda)\phi'(h(\vec{x}_i^+)) -  \lambda\phi'(h(\vec{x}_i^-))\notag\\
    &\quad~~~~~~~~~ - \frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} (\lambda -h(\vec{x}_i))\phi'(h(\vec{x}_i)) + \phi(h(\vec{x}_i)), \label{eq:empirical-bregman-decomposition}
\end{align}
where $\mathfrak{C} = \expect{Y}{\phi(Y)}$. Again, $\mathfrak{C}$ can be considered as a constant and ignored in the optimization process. From \eqref{eq:empirical-bregman-decomposition}, we can see that unbiased estimator $\hat{R}$ contains one free parameter $\lambda$, which can be tuned to minimize the variance in the estimator \citep{Sakai2017,Bao2018}. As in \citet{Sakai2017}, we show the optimal $\lambda$ when $n_\unlabeled \to \infty$ as follows.

\begin{thm}\label{thm:optimal-lambda-in-uniform}
For given regression function $h$, let $\sigma^2_+, \sigma^2_-$ be 
\begin{align*}
    \sigma^2_+ = \Var{\vec{X}^+}{\phi'(h(\vec{X}^+))}, \quad \sigma^2_- = \Var{\vec{X}^-}{\phi'(h(\vec{X}^-))}, 
\end{align*}
respectively, where $\Var{\vec{X}}{\cdot}$ denotes the variance on the random variable $\vec{X}$. Then, setting
\begin{align*}
    \lambda = \frac{\sigma^2_+}{\sigma^2_+ + \sigma^2_-}
\end{align*}
yields the estimator with the minimum variance among estimators in the form of \eqref{eq:empirical-bregman-decomposition} when $n_\unlabeled \to \infty$.
\end{thm}

Now, we establish an estimation error bound of $\hat{R}$ based on pseudo-dimension \citep{Haussler1992}. Let $\mathcal{H}$ be the hypothesis space, and we consider the following two pseudo-dimensions.
\begin{align*}
    &\tilde d = \mathrm{Pdim}(\{\vec{x} \to \phi'(h(\vec{x})) ~|~h \in \mathcal{H}\}),\\
    &\tilde d' = \mathrm{Pdim}(\{\vec{x} \to (1-\lambda-h(\vec{x}))\phi'(h(\vec{x})) + \phi(h(\vec{x}))~|~h \in \mathcal{H}\}),
\end{align*}
where $\mathrm{Pdim}(\mathcal{F})$ denotes the pseudo-dimension of the functional space $\mathcal{F}$. Assuming $\tilde d, \tilde d'$ are finite, the estimation error bound of $\hat{R}$ can be shown as follows.
\begin{thm}\label{thm:uniform-generalization-bound}
Suppose that $\tilde d, \tilde d'$ are finite and $|\phi(h(\vec{X}))|,|\phi'(h(\vec{X}))|$ are bounded, i.e., there exist constants $m,M$ which satisfy $|\phi(h(\vec{X}))| \leq m, |\phi'(h(\vec{X}))| \leq M$ for all $\vec{X} \in \mathcal{X}$. Then, we have 
\begin{align*}
    R(\hat{h}) \leq R(h^*) + O\left(\sqrt{\frac{\log 1/\delta}{n_\unlabeled}}\right) + O\left(\sqrt{\frac{\log 1/\delta}{n_\rank}}\right)
\end{align*}
with probability $1-3\delta$, where $h^*, \hat{h}$ are the minimizers of \eqref{eq:expected_loss} and \eqref{eq:empirical-bregman-decomposition} in hypothesis space $\mathcal{H}$, respectively.
\end{thm}

Note that the conditions of bounded $|\phi(h(\vec{X}))|,|\phi'(h(\vec{X}))|$ are not strict when the target variables are marginally distributed uniformly since $\mathcal{Y} = [0,1]$. From Theorem~\ref{thm:uniform-generalization-bound}, we can see that minimizing $\hat{R}$ yields the consistent regression function, i.e., $R(\hat{h}) \to R(h^*)$ as $n_\unlabeled \to \infty$ and $n_\rank \to \infty$. The convergence rate is $O(1/\sqrt{n_\unlabeled}+1/\sqrt{n_\rank})$, which is the the optimal parametric rate for
the empirical risk minimization without additional assumptions \citep{Mendelson2008}.



\begin{comment}
Let us introduce two additional random variables, $\vec{X}^+, \vec{X}^-$, which are defined as
\begin{align}
    \vec{X}^+ = \begin{cases}
    \vec{X} & (C = 1),\\
    \vec{X}' & (C = -1),\\
    \end{cases}
    \quad 
    \vec{X}^- = \begin{cases}
    \vec{X}' & (C = 1),\\
    \vec{X} & (C = -1),\\
    \end{cases} \label{eq:def_X_compare}
\end{align}
where random variables $(X,X',C)$ follow the distribution of pairwise rank data. Intuitively, $X^+$ has the feature with the larger target value compared to $X^-$. The following lemma states the distributions that these random variables follow.

\end{comment}

\begin{comment}
Since $F_Y(y) = y$ when the marginal distribution of $Y$ coincides with uniform distribution, we can decompose expected loss \eqref{eq:expected_loss} as follows.
\begin{lem}\label{lem:bregman-decomposition}
If the marginal distribution of $Y$ coincides with the uniform distribution on $[0,1]$, we have
\begin{align}
    R(h) &= \expect{\vec{X},Y}{d_\phi(Y,h(\vec{X})}\notag \\
    %&= \mathrm{const.} - \lambda \left(\expect{\vec{X}^+}{\frac12\phi'(f(\vec{X}^+))} -\expect{\vec{X}}{f(\vec{X})\phi'(f(\vec{X})) - \phi(f(\vec{X}))}\right)\notag\\
    %&\quad  + (1-\lambda) \left(\expect{\vec{X}^-}{\frac12\phi'(f(\vec{X}^-))} -\expect{\vec{X}}{(1-f(\vec{X}))\phi'(f(\vec{X})) + \phi(f(\vec{X}))}\right)
    &= \mathfrak{C} - \frac{\lambda}{2} \expect{\vec{X}^+}{\phi'(h(\vec{X}^+))} +\frac{1-\lambda}{2} \expect{\vec{X}^-}{\phi'(h(\vec{X}^-))} \notag\\
    &\quad - \expect{\vec{X}}{(1 - \lambda -h(\vec{X}))\phi'(h(\vec{X})) + \phi(h(\vec{X}))}
    \label{eq:bregman-decomposition}
\end{align}
for all $\lambda>0$, where $\mathfrak{C} = \expect{Y}{\phi(Y)}$. 
\end{lem}
%The constant $\lambda$ is chosen to minimize the variance approximation as in \citet{Sakai2017}, though we concentrate on $\lambda = \frac12$ because of the symmetry. The empirical approximation of \eqref{eq:bregman-decomposition} is

Now, the empirical approximation of \eqref{eq:bregman-decomposition} is
\begin{align}
    %\hat{R}(f) &= \mathrm{const.} - \frac12 \left(\frac{1}{2n_\rank}\sum_{\vec{x}^+_i \in \mathcal{D}^+_\rank} \phi'(f(\vec{x}_i^+)) - \frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} f(\vec{x}_i)\phi'(f(\vec{x}_i)) - \phi(f(\vec{x}_i))\right)\notag\\
    %&~  + \frac12\left(\frac{1}{2n_\rank} \sum_{\vec{x}^-_i \in \mathcal{D}^-_\rank}{\phi'(f(\vec{x}_i^-))} -\frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} {(1-f(\vec{x}_i))\phi'(f(\vec{x}_i)) + \phi(f(\vec{x}_i))}\right), \label{eq:empirical-bregman-decomposition}
    \hat{R}(h) &= \mathfrak{C} - \frac{\lambda}{2n_\rank}\sum_{\vec{x}^+_i \in \mathcal{D}^+_\rank} \phi'(h(\vec{x}_i^+)) + \frac{1-\lambda}{2n_\rank}\sum_{\vec{x}^-_i \in \mathcal{D}^-_\rank} \phi'(h(\vec{x}_i^-)) \notag\\
    &\quad - \frac{1}{n_\unlabeled} \sum_{\vec{x}_i \in \mathcal{D}_\unlabeled} (1 - \lambda -h(\vec{x}_i))\phi'(h(\vec{x}_i)) + \phi(h(\vec{x}_i)), \label{eq:empirical-bregman-decomposition}
\end{align}
where $\mathcal{D}^+_\rank = \{\vec{x}^+_i\}_{i=1}^{n_\rank}$ and $\mathcal{D}^-_\rank = \{\vec{x}^-_i\}_{i=1}^{n_\rank}$ are datasets generated from $D_\rank = \{\vec{x}_i,\vec{x}'_i,c_i\}_{i=1}^{n_\rank}$ as follows:
\begin{align}
    \vec{x}_i^+ = \begin{cases}
    \vec{x}_i & (c_i = 1),\\
    \vec{x}'_i & (c_i = -1),\\
    \end{cases}
    \quad 
    \vec{x}^-_i = \begin{cases}
    \vec{x}'_i & (c_i = 1),\\
    \vec{x}_i & (c_i = -1).\\
    \end{cases} \label{eq:def_X_compare_emp}
\end{align}
We can easily see that $\vec{x}_i^+,\vec{x}_i^-$ are i.i.d. samples of $\vec{X}^+,\vec{X}^-$, respectively. We show the following generalization error bound.

\end{comment}
